Collective Autoscaling for Cloud Microservices

As cloud applications shift from monoliths to loosely coupled microservices, application developers must decide how many compute resources (e.g., number of replicated containers) to assign to each microservice within an application. This decision affects both (1) the dollar cost to the application developer and (2) the end-to-end latency perceived by the application user. Today, individual microservices are autoscaled independently by adding VMs whenever per-microservice CPU or memory utilization crosses a configurable threshold. However, an application user's end-to-end latency consists of time spent on multiple microservices and each microservice might need a different number of VMs to achieve an overall end-to-end latency. We present COLA, an autoscaler for microservice-based applications, which collectively allocates VMs to microservices with a global goal of minimizing dollar cost while keeping end-to-end application latency under a given target. Using 5 open-source applications, we compared COLA to several utilization and machine learning based autoscalers. We evaluate COLA across different compute settings on Google Kubernetes Engine (GKE) in which users manage compute resources, GKE standard, and a new mode of operation in which the cloud provider manages compute infrastructure, GKE Autopilot. COLA meets a desired median or tail latency target on 53 of 63 workloads where it provides a cost reduction of 19.3%, on average, over the next cheapest autoscaler. COLA is the most cost effective autoscaling policy for 48 of these 53 workloads. The cost savings from managing a cluster with COLA result in COLA paying for its training cost in a few days. On smaller applications, for which we can exhaustively search microservice configurations, we find that COLA is optimal for 90% of cases and near optimal otherwise.

==> comments.tex <==

Abstract:
\as{I thought we didn't have tail anymore except for 
one microbenchmark?} - We have evaluations for Train Ticket and Online Boutique with tail latency.

$F$\as{what is F here?} - Fixed, this definition got lost in shortening the section

and select the $k$ workloads\as{What is $k$ here?} with the smallest Euclidean distance to the observed workload

==> future_work.tex <==
\section{Limitations and Future Work}
\label{sec:future-work}

We have presented a learned approach to cluster autoscaling in Kubernetes that prioritizes user experience and developer economics rather than machine utilization. The experiences from building this system sheds light on future work that can give deeper insight into the autoscaling problem and leverage the techniques presented for similar challenges.

A few system improvements may yield a more granular picture of microservice performance. Firstly, incorporating trace level information \cite{sigelman2010dapper, OpenZipk7:online, Jaegerop26:online} -- which include per hop information for requests within a microservice cluster -- adds lower level information compared to aggregate request latency which optimization algorithms such as ours could possibly take advantage of. Secondly, some algorithms can exploit correlations between coordinates of a bandit action space. Doing so in our case, and using these correlations to scale groups of microservices without human intervention could make optimization faster.

% In training our optimization models, we build a mapping between a given workload and the necessary resources required to meet the workload. This information can be generally useful in determining code efficiency in production deployments. In a continuous integration and continuous delivery pipeline, code is built, tested and deployed through automated tools typically provided by source code management platforms \cite{github:online, gitlab:online}. While such systems often test for code correctness, efficiency is contextual and in some cases it may be difficult to realistically measure. A developer using \sysname can evaluate workload resource requirements and cross reference the performance against previous models for earlier versions of the same codebase.

Lastly, more extensively examining \sysname{} across more workloads and applications would help give further insight into the scaling decisions made. Evaluating on larger microservice applications and deploying microservices with several pods per node is planned for future work.

==> intro.tex <==
\section{Introduction}
Cloud applications are increasingly built out of loosely coupled microservices communicating over RPCs\cite{netflix-ms:online, twitter-ms:online, uber-ms:online}. Building applications out of microservices allow teams in large organizations to independently develop code with fewer concerns about programming language choice and code dependencies. This reduces friction in software development. However, this flexibility and modularity complicates autoscaling: automatically allocating compute resources to each microservice as the application and its workload change. Today, individual microservices in an application are autoscaled independent of other microservices using autoscalers provided by cluster managers like Kubernetes, which scale up/down each microservice when a specific CPU/memory utilization threshold is crossed. But this approach has multiple drawbacks.

First,  {\em the ultimate goal is to cost effectively meet an end-to-end latency target (e.g. median latency $\leq$ 50ms) for the overall application---not to meet a latency or utilization requirement for any individual microservice.} Meeting an end-to-end latency goal requires carefully setting different utilization thresholds for each microservice because each microservice's demand for compute resources differs depending on its application logic. In essence, a single operator must know the internals of all microservices~\cite{gan2020unveiling}, negating the benefits of loose coupling. Second, because microservices call each other, scaling one microservice up/down can affect the time spent by a user request at a {\em different microservice}, e.g., due to backpressure, queues on one microservice cause more queues upstream \cite{zhang2021sinan}. Third, the microservice architecture allows rapid iteration of each microservice, but adding a feature or fixing a bug in one microservice might necessitate updating utilization thresholds for multiple microservices. Fourth, the utilization thresholds needed to meet a latency target depend on the workload the application receives (\S\ref{subsec:dda}).

We introduce \sysname{}: Constraint Optimizing Learned Autoscaler. Developers give \sysname{} an application, a range of workloads, and an end-to-end latency target. During training (\S\ref{sec-design}), \sysname{} efficiently samples different allocations of VMs to microservices to learn which allocations meet the latency constraint while minimizing dollar costs. After training, \sysname{} operates as an online controller (\S\ref{sec-implementation}): it monitors an application's workloads, queries for similar trained workloads, and then applies the VM allocations associated with those workloads. In summary, \sysname{} learns economical cluster configurations which meet end-to-end latency targets.

\sysname{} employs 2 key ideas during training. First, it selects those microservices that most negatively impact end-to-end latency, i.e., those that see the highest increase in CPU utilization under the given workload. Empirically, giving these microservices additional VMs often significantly reduces  end-to-end latency (\S\ref{subsec:deconstruct-cola}). Second, for the selected microservice, \sysname{} uses a multi-armed bandit to set the number of VMs to optimize a reward metric, which captures a tradeoff between meeting an end-to-end latency target and paying for more VMs. \sysname{} iterates on this selection-optimization loop until the latency target is met.

We evaluated \sysname{} on 5 open source Kubernetes microservice applications including the largest available open source application in terms of number of microservices~\cite{zhou2018poster}. We perform these evaluations on the public cloud through the Google Kubernetes Engine (GKE) platform. We compare \sysname{} against the cheapest of five machine learned and utilization based autoscalers which receive a similar level of application information as \sysname{}. Concretely, \sysname{} is compared against the best of five alternative policies -- two CPU based autoscalers (one with 30\% and another with 70\% utilization threshold) and three machine learning baselines from literature which we re-implement. These machine learning baselines apply different techniques in resource management including linear regression (inspired by Ernest \cite{venkataraman2016ernest}), Bayesian optimization (inspired by Cherry Pick \cite{alipourfard2017cherrypick}) and Deep Q-Learning models (inspired by FIRM \cite{qiu2020firm}).


Across 31 of 39 workloads where \sysname{} meets a desired latency target, \sysname{} reduces cost of microservice deployment by 30.9\% when compared to the next cheapest autoscaler across our 5 baselines. We describe these workloads in detail in our evaluation section (\S\ref{sec-evaluation}) but at a high level these include constant rate, diurnal and randomly sampled rates. For these workloads, Table \ref{tab:summary-table} shows \sysname{}'s cost reduction broken down by application. Across the 4 workloads where \sysname{} is not the most cost effective autoscaler it is, on average, 9.6\% more expensive than the cheapest autoscaler which meets the desired latency target. The lowest cost policy which meets the corresponding latency target on the remaining 8 workloads costs 66.7\% more than \sysname{}. Further, we evaluate and find that \sysname{} outperforms baselines on a set of different compute environments where we vary node size and cluster type. A full set of tabular results is provided in Appendix Tables \ref{tab:bi-fr-tabular}-\ref{tab:tt-ap-tabular}.

% Out of the 6 workloads where \sysname{} misses the latency target, half are cases where \sysname{} misses by 6\% of the latency target or less. 
\begin{table}[H]
  \begin{tabular}{lll}
    \toprule
    Application& Microservices & Cost Reduction \\
    \midrule
  Simple Web Server \cite{sws:online}  & 1 &  49.56\%\\
  Book Info \cite{binfo:online} & 4 &  19.19\% \\
  Online Boutique \cite{ss:online} & 11 &   53.06\%\\
  Sock Shop \cite{ob:online} & 14 &  1.34\% \\
  Train Ticket \cite{zhou2018poster} & 64 &   52.28\%\\
  \bottomrule
\end{tabular}
\caption{\sysname{} Cost Reduction compared to next best Autoscaling Policy from 2 CPU threshold autoscalers and 3 machine learned autoscalers}
\label{tab:summary-table}
% \vspace{-0.25cm}
\end{table}

In summary, our contributions are:
\begin{CompactEnumerate}
%    \item We formalize the problem of autoscaling microservices in a cloud setting and show how this problem can be cast as a learning problem.
    \item We design and implement \sysname{}, a learned autoscaling system which optimizes autoscaling policies for dollar cost, while meeting an end-to-end latency target. \sysname{} tailors these policies to particular applications and workloads.
    \item We evaluate \sysname{} using a range of microservice applications and workloads. Our evaluations show that \sysname{} learns policies that meet end-to-end latency targets while saving developers between 1.34-52.28\% of their dollar cost (as seen in Table \ref{tab:summary-table}).
    \item We demonstrate that initial training costs for \sysname{} are paid for by the cost savings of deployment in less than one day in some cases and within a week for most cases. Additionally, we find \sysname{} can be incrementally retrained for new latency targets and workloads with small overhead. 
    % Add specific numbers here for more items.
\end{CompactEnumerate}

==> old_text/abstract.tex <==
%We discuss several optimizations, inspired by systems and machine learning literature, we make during training to efficiently explore the space of possible microservice configurations. These optimizations enable us to train our models over the course of a few hours.

% Developers of cloud microservices are tasked with determining resources needed for their application. This choice typically relies on using either machine utilization (e.g. CPU, RAM) metrics or machine learned policies. We design, implement and evaluate microservice autoscalers that \textit{efficiently} learn to manage cluster resources based on user provided end-to-end latency targets and cost objectives. 

% We design, implement and evaluate a microservice autoscaling system, COLA, which \textit{efficiently} learns to manage cluster resources based on user provided end-to-end latency targets and cost objectives rather than optimizing utilization metrics.

% Our approach, \sysname{}, relies on training a contextual multi armed bandit on representative workloads for an application and uses techniques to generalize performance to unseen workloads. We evaluate workloads of varying complexity including those with a fixed rate, diurnal pattern and dynamic request distribution. Across a set of five open-source microservice applications, we compare \sysname{} against a variety of utilization and machine learning baselines. We
% find \sysname{} provides the most cost effective autoscaling solution for a desired median or tail latency target on 13 of 18 workloads. On average, clusters managed by \sysname{} cost 25.1\% fewer dollars than the next closest alternative that meets a specified target latency. We discuss several optimizations, inspired by systems and machine learning literature, we make during training to efficiently explore the space of possible microservice configurations. These optimizations enable us to train our models over the course of a few hours. The cost savings from managing a cluster with \sysname{} result in the system paying for its own training cost within a few days.

% Lastly, we examine the autoscaling choices being made to better understand how performance improvements are realized and examine the robustness of our learned policies.

% A broad class of autoscalers for the microservice setting predict or react to machine utilization, typically CPU or memory utilization. 

==> old_text/background.tex <==
% \begin{figure*}[!t]	
% 	\centering
% 	\includegraphics[width=.31\textwidth]{figs/updated/allocations/bi_hpa.pdf}
% 	\caption{Horizontal Pod Autoscaler - Latency vs. # of VMs for Book Info Application}
% 	\includegraphics[width=.31\textwidth]{figs/updated/allocations/ob_hpa.pdf}
% 	\includegraphics[width=.31\textwidth]{figs/updated/allocations/ob_traces.pdf}
% 	\caption{Effects of utilization based Horizontal Pod Autoscaling on microservice applications. Latency vs. Total Number of replicas for Book Info \cite{binfo:online} (left) and Online Boutique \cite{ob:online} (center). Constant rate workload applied for 5 mins for 5 different target CPU utilizations from 10-90\%.}
% 	\label{fig:hpa-evals}
% \end{figure*}

% Equipped with the above tools to scale the resources of a Kubernetes cluster, users may optimize the performance and dollar cost of their microservice. We now discuss how automatic scaling, also known as autoscaling, policies are typically deployed in Kubernetes.

%\Para{Common Approaches} Based on a survey of tens of thousands of Datadog \cite{DdogContainerReport:online} customers running more than 1.5 billion containers, it is estimated that 90\% of organizations running Kubernetes clusters are doing so through managed services offered by cloud providers. Additionally, roughly 40\% of organizations leverage Horizontal Pod Scaling while just 1\% use Vertical Pod Scaling. 
% These Pods are configured and are deployed and managed through a command line interface to the Master Node.

% Secondly, Google details the container autoscaling approach used internally called Autopilot \cite{rzadca2020autopilot}. Serving jobs, which comprise the bulk of compute resources within Google, generally aim to meet strict performance guarantees on end to end response time (e.g. a latency objective of $\leq$ 50ms). These jobs are observed to have diurnal or weekly patterns which may change more significantly over longer time horizons as code changes and services rise or fall in popularity. Serving jobs use Horizontal Pod Autoscalers which are scaled either by hand tuned rules or with CPU or Memory utilization based metrics.

% In this paper, we examine, design and evaluate autoscaling policies for Horizontal Pod Autoscaling (HPA). We now discuss the specific implementation of Kubernetes' HPA as well the implementation used by Autopilot \cite{rzadca2020autopilot} -- utilization threshold based HPA.
% on the most common setting for application developers by developing and benchmarking Horizontal Pod autoscalers which run on managed Kubernetes clusters.

%%%>>>>>>>>>>>>>>>>>>>>>>>>

% In the following subsection, we discuss how the choice of target utilization value effects both the cost and latency of a microservice application. Further, we discuss the challenges in deploying this class of autoscaling policy.

% The total desired replicas, and consequently the total compute resources, are aggregated across all microservices.

% Throughout this paper, we evaluate on 
% While several evaluation settings could be considered, surveys from cloud monitoring organizations suggest the most  is the most common setting for application developers. 

% 2. Describe the shortcomings of the approach
    % Selecting correct threshold for a given workload is not obvious
    % Depending on the workload, the threshold changes
    % Marginal benefits of scaling each service vary as a function of the actual SLO. Each autoscaling threshold is set on a service based, does not correspond to SLO.
    
% \subsection{Queuing Models}

% In many cases, analyzing the state of system queues can help application developers understand how and when to react to workloads by altering resource management strategies. However, and as has been noted by others, microservice based systems prove to be a challenging setting for such analysis \cite{zhang2021sinan}. 

% Specifically, requests entering a microservice pass through what can be thought of as a sequence of multi-server queues. For the purpose of analysis, let us assume that our microservice graph is acyclic, leading to a fixed input rate to one such service, $i$, which we would like to optimize. Further, let us assume that the workload is equally distributed across all replicas of this service and that requests never time out.  We let $c_i$ represent the number of replicas of service $i$, $\lambda_i$ the (Poisson) arrival rate, $\mu_i$ the service rate of the workload and $\rho_i$, the utilization of the queues, is equal to $\frac{\lambda_i}{\mu_i}$.


% To obtain queuing probability for service $i$, we can use Erlang's C formula \cite{kleinrock1975queueing}, which models the probability a packet will wait in our multi server queue.

% \begin{equation*}
%     \label{equation:erlang-c-prob-wait}
%     C(c, \rho) = \frac{\frac{\rho^c c}{c! (c-\rho)}}{\sum_{n=0}^{c-1} \frac{\rho^n}{n!} + \frac{\rho^c c}{c! (c-\rho)}}
% \end{equation*}

% % For the above model, the wait probability is dependent on the number of replicas of a service, $c$, and $\rho$ -- the ratio of the (Poisson) arrival rate to the queue, $\lambda$ and the service rate of the workload $\mu$.

% We can then obtain the following average latency $W_i$ for service $i$, where $c_i$ represents the number of replicas of service $i$, $\lambda_i$ is the (Poisson) arrival rate, $\mu_i$ is the service rate of the workload and $\rho_i = \frac{\lambda_i}{c\mu_i}$.

% \begin{equation*}
%     \label{equation:erlang-c}
%     W_i(c_i, p_i, \mu_i) = \frac{1}{\mu_i} + \frac{1}{\mu_i(c_i-\rho_i)\cdot C(c_i, \rho_i)}
% \end{equation*}

% In order to carry this analysis forward for an application with multiple microservices we can model the system as a connected sequence of multi server queues. However, to do so we must have knowledge on the input and output rates of each class of multi-server queues for every microservice and the probabilities of moving from one microservice to another. Further, even for the case with one multi server queue, we have made assumptions that requests are distributed according to a Poisson random variable, that queue sizes can grow indefinitely and that requests are evenly distributed across servers.
% % Mention the specific assumptions

% % We draw inspiration from this multi-server queueing model to design a few heuristics in \sysname. 
% Impracticality both in terms of required application knowledge and assumptions on our workload and system encourage us to explore another avenue for optimizing microservice clusters: \textit{data-driven autoscaling}. We now require an algorithm to help explore and select a good cluster configuration for a given workload, which we describe now.


% % % % % % % % % % % % % % % % 
% TO DO
% % % % % % % % % % % % % % % % 
% 1. MAB algorithm - done
% 2. Clean up Contextual Bandit







% 

% Objective

% Context


% \subsection{Multi-Armed Bandits}
% \label{subsec:mab}

% % Multi-Armed Bandit procedure
% \Para{Multi-Armed Bandit Procedure}
% The multi-armed bandit framework outlines an approach to selecting an optimal action across a set of actions in order to maximize some expected reward. An agent making this determination of an optimal action can sample the reward for any given action but has the goal of finalizing an optimal action with as few samples as possible. 

% Concretely, let us assume we have $A$ possible actions (a.k.a. \textit{arms}) to choose from and $T$ total trials where we may sample any one arm $a \in A$. Each arm $a$ produces a reward which we model as an IID sample from $D_a$, the arm's corresponding real-valued distribution over rewards. We assume that the reward per sample is bounded. As we assume the only knowledge we are given is the set of arms $A$ and a number of trials $T$, we must sample the arms to infer which action produces the highest expected reward. A simple algorithm, shown below in Algorithm \ref{alg:uniform-bandit}, is to sample each arm $\frac{T}{|A|}$ times and select the arm with the highest average reward once our trial budget is exhausted.


% \begin{algorithm}
% \caption{Uniform Bandit}\label{alg:uniform-bandit}
% \begin{algorithmic}[1]
% \For{$a \in A$}
%     \State $N_a = \epsilon$
%     \State $R_a = 0$
% \EndFor
% \For{$t=1,2,...,T$}
%     \State Select $a_t = \argmin_{a \in A} N_a$ \Comment{Break ties randomly}
%     \State Observe reward $R_t$ for action $a_t$
%     \State $N_a = N_a + 1$ 
%     \State $R_a = R_a + \frac{R_t - R_a}{N_a}$
% \EndFor
% \State \textbf{return} $\argmax_{a \in A} R_a$
% \end{algorithmic}
% \end{algorithm}


% % Contextual bandit formulation
% % \Para{Contextual Bandit Procedure}
% % % Contextual Bandit description
% % % Connect this quickly to our problem
% % The contextual bandit extends the multi-armed bandit setting by allowing the agent to observe some contextual information presented by the environment before selecting an action. This context, which we denote as a vector $x_t \in \mathbb{R}^d$, may include information regarding each of the actions along with other information which may be useful for reward determination. For example, a workload's number of requests per second issued to a microservice application may be useful when determining what action, the number and type of nodes in a cluster, to select. Leveraging this context, the bandit may learn to customize cluster configurations based on specific workload details. This contextual bandit procedure is shown in Algorithm \ref{alg:contextual-bandit}.

% % % In the contextual bandit framework, an algorithm $B$ conducts a series of trials $t=1,2,3,..., T$.


% % \begin{algorithm}
% % \caption{Contextual Bandit Training}\label{alg:contextual-bandit}
% % \begin{algorithmic}[1]
% % \For{$t=1,2,...,T$}
% % \State Receive context $x_t$
% % \State Select action $a_t = \argmax_{a \in A_t} f_t(x_t, a)$ \Comment{E.g. Equation \ref{eq:select-arm}}
% % \State Observe reward $r_t$
% % \State Update $f_t$ given ($a_t, r_t, x_t$)
% % \Comment{E.g. Equation \ref{eq:update-theta}}
% % \EndFor
% % \State \textbf{return} $f_T$
% % \end{algorithmic}
% % \end{algorithm}


% % % \begin{CompactEnumerate}
% % %     \item The algorithm receives: $u_t$ - the contextual information regarding the state presented at time $t$ and $A_t$ the set of possible actions. The features for the workload and actions are provided as a vector for each action $x_{t,a}$ for each action $a \in A_t$.
% % %     \item Based on the historical reward observed in previous trials, $B$ selects an arm $a_t \in A_t$ and receives the reward $r_{t, a_t}$ which is a function of both $u_t$ and $a_t$.
% % %     \item Recognizing this reward, $B$ improves its arm-selection strategy with new information $(x_{t,a_t}, a_t, r_{t, a_t})$.
% % % \end{CompactEnumerate}

% % One common way to use contextual information is by constructing a linear contextual bandit. For this construction, the linear contextual bandit selects an arm by constructing a linear map, $\theta_a$, between the context, $x_{t,a_t}$ and the observed trial payoffs $r_{t, a}$. Such models assume that the expected reward is linear with respect to the features contained in the context. 

% % $$ E[r_{t,a} | x_{t,a}] = x_{t,a}^T \theta_a$$


% % Given some set of weights $\hat{\theta}$, we can  select the action that maximizes the expected reward for a presented context, $x_{t,a}$, with a linear function as follows.

% % \begin{equation}
% %     \label{eq:select-arm}
% %     a_t \triangleq \argmax_{a \in A_t} x_{t,a}^T \hat{\theta}_a
% % \end{equation}

% % There are several ways to estimate our weights, $\hat{\theta}$. As an example, we can do so by solving an ordinary least squares problem. Let $X_a$ represent the concatenated set of $T$ training example contexts where action $a$ was selected. Also let letting $R_a$ represent the concatenated set of rewards for each of those examples. We can now estimate $\hat{\theta}_a$ for each action $a \in A$ by solving the following system of linear equations.

% % \begin{equation}
% %     \label{eq:update-theta}
% %     \hat{\theta}_a = (X_a^TX_a)^{-1} (X_a^{T}R_a)
% % \end{equation}

% % % Arm selection
% % % FIX



% \Para{Objective and Evaluation Metrics}
% The goal of algorithm $B$ is to maximize the \textit{cumulative reward}, $\sum_{t=i}^{T} r_{t, a_t}$, throughout its training process. If the optimal action for each trial is known, we can also compute the \textit{regret} of the bandit which is the difference between the cumulative reward for an optimal algorithm and $B$.


% % FIX
% % $$ R_{B}(T) \triangleq E\bigg[\sum_{t=i}^{T} r_{t, a^{*}_t}\bigg] - E\bigg[\sum_{t=i}^{T} r_{t, a_t}\bigg]$$


% % Reasoning for the model
% % In the autoscaling context, we represent the user as the number of requests per second issued to our microservice. The set of actions is represented as the number of pod replicas for a given microservice. 


% % Tighten up reasoning + introduce interpolation based bandit ?




% \subsection{Model Predictive Control (Update -> Contextual Bandits)}
% Many control techniques may be applied to optimize cluster scale given performance and cost constraints. We choose to leverage Model Predictive Control (MPC) as the method facilitates the use of a broad class of predictive models ranging in complexity from linear models to deep neural networks. This flexibility allows users to select a predictive model that offers the right trade-off between model interpretability and expressivity. 

% We briefly review MPC and refer readers to \cite{camacho2013model} for a more detailed treatment along with theoretical derivations.

% \subsubsection{Formulation}

% % (todo) Check to make sure this notation matches same vars used in common literature.
% MPC is a control technique which optimizes the state $X \in \mathbb R^n$ of a system subject to forecasted future inputs $U \in \mathbb R^m$ to a system. We observe these states and inputs at discretized, uniform time steps $t \in T$. 

% The approach relies on building two models: firstly a predictive model of the input process, $\phi: \mathbb R^m \rightarrow \mathbb R^m$, and secondly a cost function between an input, state pair for a system, $\ell: \mathbb R^n \times \mathbb R^m \rightarrow \mathbb R$.

% These predictive models can be arbitrary, although we traditionally refer to techniques that use linear models as Linear MPC and those that use nonlinear models as Nonlinear MPC. Often, historical data on inputs and states are collected to empirically fit these models.

% Given models $\phi$ and $\ell$, we can formulate an optimization problem which chooses the best future state for a horizon of future time steps subject to problem and/or user constraints.

% \begin{equation}
% \begin{aligned}
% \min \quad & \sum_{\tau=t}^{t+T}\ell(x(\tau), u(\tau))\\
% \textrm{subject to} \quad & u(\tau) \in U, \; x(\tau) \in X  \quad \tau= t,..., t+T\\
%   & u(\tau+1) = \phi(u(\tau))\\
% \end{aligned}
% \end{equation}
% Solving this problem yields a plan for the next $T$ steps, $x(t), ..., x(t+T)$. At each time step we apply our control for the next time step only, $x(t)$, and continue this process forward.

==> old_text/conclusion.tex <==
\section{Conclusion}
\label{sec-conclusion}

\sysname{} is an autoscaling system that learns to optimize microservice clusters efficiently from experience. \sysname{} performs various optimizations to search the possible space of microservice configurations subject to user driven constraints and provided workloads. Once trained, the system leverages experience to manage clusters in real time, amortizes it's training cost and importantly is robust to several sources of inevitable noise and failure. \sysname{} is able to offer performance nearing or matching the requirements set by users in all workloads we evaluate. We compare \sysname{} against the best selected utilization and machine learned autoscaling policy, which differ depending on the application and workload. \sysname{} matches or outperforms the best competing policies for 13 out of 18 workloads and reduces microservice cluster cost by 25.1\% on average. \sysname{} achieves these results with little human effort, application knowledge, and system dependencies.
%We hope that our discussion of \sysname{} can prompt further examination in learning-based autoscaling for microservice applications.


% Implications beyond this paper

% Prompt further approaches towards learning from experience
% Make a note of google scholar based search results

% Further, \sysname{} is within 10\% of the cost of the best policy on workloads where it is outperformed.

%A few extensions we believe are worth highlighting include predictive autoscaling, the integration of autoscaling and scheduling algorithms, and leveraging finer grained metrics from microservice tracing tools. First, given that workloads often vary predictably across some time (daily, hourly, weekly, etc.), it may be feasible to predict the request rates of the near future. Then, for example, from these predictions we may be able to make updates to our cluster in anticipation of an increase or decrease in requests. Second, our evaluations involve cluster setup in which microservices are not co-located on the same virtual machine. While this reduces noise from noisy neighbor effects, this cluster setup is inefficient in its use of resources for some applications. Modifying \sysname{} to additionally make scheduling decisions, for example in terms of the affinity of two types of microservices, can potentially further reduce latency by allowing frequently communicating microservices to co-locate. Third, integrating measurements from tracing tools to better understand the time requests dwell at each microservice can potentially help more efficiently search for autoscaling policies.


%While we have presented an approach to efficiently search for autoscaling policies, finer grained measurements may yield better estimates of which services are a bottleneck for an application or a more efficient search routine across autoscaling policy candidates. 


%The novelties described above are aimed at satisfying a few key design decisions: broad applicability across applications and workloads and robust performance if/when such a system runs in production. To accomplish this first goal, we do not assume any software beyond a load balancer which is provided as a managed service from large cloud providers. Additionally in Section \ref{subsec:model-robustness}, we evaluate across a diverse set of applications with several workloads to confirm our approach works well broadly. In pursuit of the second goal, we carry out experimentation to understand sources of control loop noise in terms of feedback delay, measurement noise and the appearance of unseen request rates and workloads.


% prioritizes user experience and developer economics rather than machine utilization. The experiences from building this system sheds light on future work that can give deeper insight into the autoscaling problem and leverage the techniques presented for similar challenges.

% A few system improvements may yield a more granular picture of microservice performance. Firstly, incorporating trace level information \cite{sigelman2010dapper, OpenZipk7:online, Jaegerop26:online} -- which include per hop information for requests within a microservice cluster -- adds lower level information compared to aggregate request latency which optimization algorithms such as ours could possibly take advantage of. Secondly, some algorithms can exploit correlations between coordinates of a bandit action space. Doing so in our case, and using these correlations to scale groups of microservices without human intervention could make optimization faster.

% In training our optimization models, we build a mapping between a given workload and the necessary resources required to meet the workload. This information can be generally useful in determining code efficiency in production deployments. In a continuous integration and continuous delivery pipeline, code is built, tested and deployed through automated tools typically provided by source code management platforms \cite{github:online, gitlab:online}. While such systems often test for code correctness, efficiency is contextual and in some cases it may be difficult to realistically measure. A developer using \sysname can evaluate workload resource requirements and cross reference the performance against previous models for earlier versions of the same codebase.

% Lastly, more extensively examining \sysname{} across more workloads and applications would help give further insight into the scaling decisions made. Evaluating on larger microservice applications and deploying microservices with several pods per node is planned for future work.

==> old_text/design.tex <==

% Then, in Section \ref{sec-design} we discuss how to efficiently search for 

% To do so we discuss how to contextualize the autoscaling policy we have based on the workload observed and secondly we formalize a reward function which dictates a ranking of autoscaling policies given a context. 


% These policies are given access to microservice applications as well as the workloads these applications typically experience. As a result, these data driven autoscalers are able to target specific end to end latencies and adjust their resource allocation strategies depending on the currently observed workload.



% ---------------

% \subsubsection{State} Let us consider an application with $D$ different microservice deployments (e.g., database, web server, cache). Each deployment, $i$, has a defined range of number of replicas which may be launched from 1 to $N_i$. We denote $N_i$ as the replica range for the deployment $i$.

% We define the state of the cluster, $S$ as a vector of number of current deployments for microservices in our application. If we consider the maximum replicas to be $N$ for all $D$ deployments, the possible states for our microservice application is $S \in \{1, 2, 3, ... ,N\}^D$.

% \subsubsection{Actions} Our model has the ability to take actions that modify the number of replicas in our cluster for each microservice to any value in its replica range, consequently altering state $S$.

% The set of all possible actions $A$ is simply the set of cluster states, $S$. At any given time a model may choose to change the cluster state to any possible configuration.


% \subsubsection{Context}
% Lastly, we formally construct a representation of a workload and denote this representation as a context $C$. This context $C$, contains information on the inbound requests to our application and serves to distinguish the workloads an application may observe. 

% % There are a variety of ways to characterize the inbound requests for an application such as including the number of requests, their URLs, headers, etc.

% In recent years, standards have been introduced by the OpenTracing \cite{opentracing:online} and OpenAPI \cite{openapi-3-1-0:online} organizations to define requests into a distinct set of "operation" names. Roughly speaking, the best practice denotes an operation as a distinct URL without its request parameters. For example, \url{get_account_by_id/id1} and \url{get_account_by_id/id2} both fall under the \url{get_account_by_id} operation name. 

% Several popular logging, monitoring and debugging tools can both propogate and utilize these specified operation names. For example microservice tracing tools (e.g. \cite{Jaegerop26:online}, Zipkin \cite{OpenZipk7:online}, and DataDog \cite{datadog:online}) annotate logs of invoked requests with their associated operation name. Monitoring and debugging tools often allow users to filter, process and analyze requests broken down by operation name.

% During training and evaluation, we assume that developers have defined $U$ distinct operations for their application. We then construct a context vector $C$ of length $U$ by concatenating the number of requests per operation name. Each element in our context vector $C_i$ is simply the number of requests to our cluster with the operation name $i$.


% % which is provided by the application developer. Also, we discuss the computation of total virtual machines given state $M_s$ in Section \ref{subsubsec-eval-settings}. Our reward for \sysname{} is defined below.

% % FIX


% % \Para{Weight Intuition} Given our reward formulation, the user now faces the burden of choosing weights to characterize how well cluster states accommodate a workload. 

% \subsubsection{Multi Armed Bandit Algorithm}



% We approach this problem with the multi-armed bandit framework. This framework outlines an approach to selecting an optimal action across a set of actions in order to maximize some expected reward. An agent making this determination of an optimal action can sample the reward for any given action but has the goal of finalizing an optimal action with as few samples as possible. Given a workload, the bandit algorithm identifies a cluster state which yields the highest reward is shown in Algorithm \ref{alg:ucb1-bandit} below. 
% % Add citation to UCB1
% % We make use of the popular UCB1 variant of the multi armed bandit framework.


% ---------------


% \begin{algorithm}
% \caption{UCB1 Bandit}\label{alg:ucb1-bandit}
%   \begin{algorithmic}[1]
%     \BlankComment{}
%     \Function{ucb}{$A, l_{target}, W$}

%     \For{$a \in A$}\Comment{Iterate over all cluster states.}
%         \State $N_a = \epsilon$ \Comment{Number of times state $a$ is sampled.}
%         \State $R_a = 0$ \Comment{Average reward for state $a$.}
%         \State $L_a = 0$ \Comment{Average latency for state $a$.}
%     \EndFor
%     % \LineCommentCont{Observe reward for each action and update average rewards.}
%     \For{$t=1,2,...,F$}
%         \State $a_t = \argmax_{a \in A} R_a + \frac{\sqrt{2log(t)}}{N_a}$ \Comment{Action for trial $t$.}
%         \State Update cluster replicas based on action $a_t$
%         \State Compute total replicas/VMs $M$ used for action $a_t$
%         \State Observe latency $L_t$ for action $a_t$
%         \State $R_t = min((l_{target} - L_t), 0) - M \cdot w $
%         % \State Observe reward $R_t$, latency $L_t$ for action $a_t$
%         \State $N_{a_t} = N_{a_t} + 1$ 
%         \State $R_{a_t} = R_{a_t} + \frac{1}{N_{a_t}} (R_t - R_{a_t})$
%         \State $L_{a_t} = L_{a_t} + \frac{1}{N_{a_t}} (L_t - L_{a_t})$
%     \EndFor
%     \State $a_{opt} = \argmax_{a \in A} R_a$ \Comment{Get action with highest reward.}
%     \State $l_{opt} = L_{a_{opt}}$ \Comment{Get corresponding latency.}
%     \State \textbf{return} $a_{opt}, l_{opt}$
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}
% \caption{Uniform Bandit}\label{alg:uniform-bandit}
% \begin{algorithmic}[1]
% \For{$a \in A$}
%     \State $N_a = \epsilon$
%     \State $R_a = 0$
% \EndFor
% \For{$t=1,2,...,T$}
%     \State Select $a_t = \argmin_{a \in A} N_a$ \Comment{Break ties randomly}
%     \State Observe reward $R_t$ for action $a_t$
%     \State $N_a = N_a + 1$ 
%     \State $R_a = R_a + \frac{R_t - R_a}{N_a}$
% \EndFor
% \State \textbf{return} $\argmax_{a \in A} R_a$
% \end{algorithmic}
% \end{algorithm}

% For our autoscaling problem we represent a workload as a distribution of requests over operation names. During training and evaluation, we assume that developers have defined $U$ operations for their application. We then construct a context vector $C$ of length $U$ by concatenating the number of requests per operation name. Each element in our context vector $C_i$ is simply the number of requests to our cluster with the operation name $i$.

% To gather these request statistics, we deploy an ingress gateway through Istio \cite{istio:online} which is instrumented to record request information including operation names for each request. Similar to microservice logging tools, Istio \cite{istio:online} provides the ability to annotate requests by operation names. This process is built in to Google Cloud Platform, the cloud provider we use for evaluations. We provide more details on this procedure in Section \ref{sec-implementation}.




% --------------------
% \subsubsection{Why use a Multi Armed Bandit?}
% The Multi Armed Bandit Framework fits the autoscaling problem well for a few reasons.

% \Para{Few Underlying Assumptions} Firstly, the model makes few assumptions on the relationship between a cluster state and its reward. Since each state is modelled seperately and initially assumed to provide equal reward (as seen in Equation \ref{alg:ucb1-bandit}), the algorithm solely relies on observed data to determine the optimal cluster state for a given workload.

% A few other choices could be to run gradient descent or binary search on the reward as a function of cluster state. However, for an optimal solution gradient descent will assume a convex relationship between reward and cluster state. Additionally, the choice of step size for gradient descent determines whether the solution converges to any optima at all. Binary search assumes the relationship between reward and cluster state is monotonically increasing or decreasing.

% \Para{Sample Efficiency} Secondly, we note that training on a microservice cluster incurs both a dollar and time cost. Finding a good set of cluster states for provided workloads are only valuable if their cost savings outweight the training cost.

% Settings in which sample efficiency is of paramount importance leverage the multi armed bandit framework. For example in A/B testing platforms \cite{optimizely:online} developers aim to determine optimal software designs in as few impressions as possible. For e-commerce recommendations developers aim to match the right product for a user with as few recommendations as possible \cite{stitchfix:online}. For drug dosing, doctors would like to make a personalized selection of the correct dosing of a drug for a patient with as few selections as possible \cite{bastani2020online}.

% % We note that one could use a reinforcement learning framework to solve the problem presented. In our setting we make the assumption that the context, or workload, is not dependent on the previous actions taken and is entirely exogenous to our system. This equates to making the assumption that the number of requests issued by users is uncorrelated with the number of machines deployed on a cluster. Aided by this assumption, we decide to forego the additional machinery and complexity that reinforcement learning would add. However, we evaluate against a deep reinforcement learning baseline in Section \ref{sec-evaluation}.
% % \sysname{} uses the bandit framework to determine high reward cluster state for a few reasons. First, the bandit framework makes few prior assumptions on the reward associated with any particular cluster state. Secondly, the framework is known to efficiently learn from few samples and as such is used in problems where samples are expensive to collect. Lastly, the algorithm is simple to implement and maintain.

% We modify the standard bandit framework for the microservice setting to reduce training cost and generalize cluster state selection to unseen workloads. In this Section we describe optimizations we make in \sysname{} which reduce training cost and time for our autoscalers. Then, in Section \ref{sec-implementation} we discuss procedures to generalize autoscaling policies to unseen workloads.

% ------------------------



% This section describes the model and training algorithm we use to learn autoscaling policies in \sysname. We present a formal description of the autoscaling problem and describe how to represent it as an learning task. We then outline optimizations we make for training which are inspired both by general literature for the multi armed bandit problem as well as specific heuristics based on our microservice autoscaling setting. We design \sysname{} to have the following qualities:

% \begin{CompactEnumerate}
%     \item \textbf{Efficient:} Microservice architectures are meant to facilitate building and updating applications with speed. \sysname{} should efficiently search the space of possible configurations and amortize its own training cost within a few days of deployment.
%     \item \textbf{Configurable:} Different developers, teams and organizations have different autoscaling goals. \sysname{} should have easily interpretable and configurable objectives and constraints over which it optimizes.
%     \item \textbf{Lightweight:} Knowledge about microservice applications can be distributed across many individuals and can become quickly deprecated. \sysname{} should make use of as little knowledge of microservice internals as possible.
%     \item \textbf{Robust:} While users may have good estimates on production workloads their applications may face previously unseen workloads. \sysname{} should be able to robustly adapt to new workloads and failover to a suitable replacement autoscaler when this is not feasible. 
% \end{CompactEnumerate}

% \begin{figure}[!t]	
% 	\centering
% 	\includegraphics[width=8cm]{figs/general/sys_diag.png}
% 	\caption{Training Setup for Bandit Autoscaler}
% 	\label{fig:training-setup}
% 	\vspace{-0.5cm}
% \end{figure}


% We formally define the state, action, reward and context of our problem below.

% We formally define the problem we address as selection a microservice configuration $M$ under a context $Y$ to maximize the expected reward $R$.

% Write more about automatically selecting weights.

% We aim to relax these evaluation settings in future work.

% We use the same weighting parameters for all but one microservice application for our evaluations. We provide the weighting parameters used for evaluations in Table \ref{tab:hyperparams}.

% study the effects of optimizing these weight parameters in Section \ref{sec-evaluation} and

% ----------------------------

% \subsection{Training Algorithm}


% From Line 6 of Algorithm \ref{alg:ucb1-bandit}, notice that evaluating the optimal action, finding $\argmax_{a \in A_t} x_{t,a}^T \hat{\theta}_a$, scales based on the size of the action space, $A$. Additionally, the space of actions $A$ available to explore are the total number of cluster states. With $D$ total deployments and assuming that we can use up to $N$ replicas per deployment, $A$ scales exponentially: $O(N^D)$.

% Microservice applications can consist of 10-100s of microservices, which makes this exponentially growing evaluation cost and exploration space especially undesirable. Our setting further exacerbates the efficient implementation of a multi armed bandit algorithm as the sampling time, the time taken to observe the reward for each sample can be lengthy. Specifically, this sampling time includes generating a workload and observing some steady state latencies of the generated workload. We find the time needed to accurately estimate steady state latency leads to a sampling duration of 30 to 60 seconds depending on the application (shown in Table \ref{tab:hyperparams}). Empirically we find that generally we can estimate the median latency within 1-2\% and the 90\%ile latency within 5\%. Evaluations of this latency estimation under several values of sampling duration are included in Section \ref{subsec:sample-duration-variation}.

% ----------------------------

% What does training involve - epsilon greedy algorithm
% During training time, contextual bandit algorithms are repeatedly presented with a context, select an action to take, and observe the reward for their selected action. This routine is shown in Algorithm \ref{alg:uniform-bandit} and discussed in Section \ref{subsec:mab}.

%  Fix this paragraph -- sampling time duration vs. error
    
% In our implementation, we create  connections to our cluster and allow time for steady state behavior for the system to be determined.

% Furthermore, we evaluate the determined action for each context which leads to cost $O(T \cdot z)$, where we let $z$ represent the time taken to evaluate an action in our microservice setting. 

% Our setting complexity
% Microservice applications can consist of 10-100s of microservices, which makes the exponential cost of determining an optimal action undesirable. This is further exacerbated as generating a load and observing the effects of this load on our microservice can be costly in terms of time. For our implementation, we create  connections to our cluster and allow time for steady state behavior for the system to be determined.

%We modify the standard multi armed bandit procedure to
%We develop a procedure to efficiently search over our state space and reduce the number of reward observations needed to find states which yield high reward for a workload.

%>>>>>>>

% \subsection{Training Optimizations}
% We make training optimizations inspired both by previous literature and our problem setting which we detail below.

%As a brief summary:
%\begin{CompactEnumerate}
%    \item In Section \ref{subsubsec:greedyhillclimbing} we break down the global search problem over all deployments to one which \textit{locally searches over a single microservice}. Doing so allows us to shrink our search space.
 %   \item In \ref{subsubsec:select-service} we discuss how to \textit{select congested services} that should be explored.
 %   \item In \ref{subsubsec:optimize-service} we discuss how we optimize the selected congested services with a \textit{multi-armed bandit model}.
%\end{CompactEnumerate}


% \subsubsection{Greedy Hill Climbing}
% \label{subsubsec:greedyhillclimbing} Several optimizations have been proposed to speed up the exploration for bandits in settings with large action spaces. A special case of this setting is multivariate optimization where each action a bandit takes can be decoupled into several separate and smaller decisions \cite{hill2017efficient}. In such cases each separate decision, such as scaling a single microservice $D_i$ for our action space, has a much smaller set of possible actions to search over, with $N_i$ possible actions, than the entire space of configurations.

% By alternating a reward maximization procedure over each of these decoupled decisions, one may obtain a locally optimal solution to searching over the entire action space by optimizing one such small decision at any given point. For example, we may optimize a single microservice for our given reward, holding the number of replicas for all other microservices as fixed. Assuming we repeat this search procedure $T$ times, we reduce the complexity of the full search from $O(N^D)$ to $O(TN)$.

% We now describe the procedures we use to select and optimize a specific microservice for each iteration of our training procedure. We repeat this process until an early stopping procedure which simply checks if the state at iteration $t$, $S^t$, meets our latency threshold and exits training if so.

% From the above reward, note that in order to obtain benefits from scaling up a cluster the reduction of latency in the service we scale should be larger than any increased latency from downstream services. We will not benefit from simply increasing queueing delays by an equal or larger amount of time at some other microservice which is not being scaled.


% We outline the algorithm we implement for autoscaling in Algorithm \ref{alg:hillclimbing}.

% \algnewcommand{\LineComment}[1]{\Statex \hskip\ALG@thistlm \footnotesize\ttfamily\textcolor{blue}{$\triangleright$ #1}}

% \begin{algorithm}
% \caption{\sysname{} Training Procedure}\label{alg:hillclimbing}
%   \begin{algorithmic}[1]
%     \BlankComment{}

%     % Outer Loop for Autoscaling Function
%     % \State{\footnotesize\ttfamily{\textbf{function} optimizeCluster($C$, $S^{0}$, $l_{target}$, $T$)}}
%     \Function{optimizeCluster}{$C$, $S^{0}$, $l_{target}$, $T$, $\lambda$, $\lambda_{max}$, $\epsilon$}
    
%         \While{$\lambda<\lambda_{max}$}
%           \For{$t=1,...,T$}
%             \State{$S^t = S^{t-1}$}
%             \LineComment{Choose a service to optimize. (Section \ref{subsubsec:select-service})}
%             % \State{$opt$ = selectService($C, S^{t}$)} 
%             \State Apply workload $C$ to cluster with state $S^{t}.$ \LineComment{Aggregate output of \texttt{kubectl top pod} by service.}
%             \State  Get $U$, list of average CPU util for each service. 
%             \LineComment{Return highest utilized service.}
%             \State $opt = \argmax_{i \in {1,...,D}} U$        
            
%             \LineComment{Optimize the chosen service. (Section \ref{subsubsec:optimize-service})}
%             \State{$S^t_{opt}, l_{opt}^t$ = ucb($A, l_{target}, W$)}
%             \If{$l_{opt} <= l_{target}$}         \State{\textbf{break}}
%             \EndIf
%           \EndFor
%           \If{$l_{opt} <= l_{target}$}         \State{\textbf{break}}
%           \Else \State{$\lambda = \lambda + \frac{1}{\epsilon}$}
%           \EndIf
%         \EndWhile
%         \State
%         \Return{$S^T, l_{opt}^t$}
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}



% \subsubsection{Single Service Reward Model}
% \label{subsubsec:queue-model} We have broken down the search at each timestep from an allocation across all deployments to one over a single deployment, while keeping all other deployments fixed, with the approach in Section \ref{subsubsec:greedyhillclimbing}. We model the problem of selecting the optimal replicas for a single deployment as one of optimizing an end to end latency of interest.

% The expected reward for this single deployment can be written in the same form as Equation \ref{equation:reward-function}, with the latency now referring to the summation of the latency for the microservice we optimize and the latency of all other services.

% We let $l_{D \setminus i}(c)$ represent the latency of all deployments excluding deployment $i$, the deployments which remain fixed during the current exploration. Our reward for scaling a single deployment can be shown as follows.

% % FIX
% \begin{equation}
% \label{equation:reward-function-single-service}
% \begin{aligned}
% R_{C, S_i} \triangleq \quad & min( l_{target} - ((l_{D \setminus i}(S_i) + l_i(S_i)) \cdot w_l, 0) \\
%   & - S_i \cdot w_s \\
% \end{aligned}
% \end{equation}

% Consequences of the queuing model
% 1. Gains depends on service we choose to optimize, reduction in latency must be larger than increased latency to other services
% 2. Non linear form for the service we scale -- depreciating marginal utility for the same marginal cost

% Secondly, the latency in our scaled service responds superlinearly to the number of instances which means that the reduction in service latency will outweigh the marginal cost for an additional replica for only some regime of instances.

% \begin{figure}[H]	
% 	\centering
% 	\includegraphics[width=8cm]{figs/bandit_reward/es_100_l.png}
% 	\caption{Bandit Latency while scaling one service across variety of workloads}
% 	\label{fig:training-setup}
% 	\vspace{-0.5cm}
% \end{figure}

% Plot of reward vs. Latency for Frontend

%>>>>>>>>>

% This procedure is shown in Algorithm \ref{alg:hillclimbing}.
% \begin{algorithm}
% \caption{UCB1 Bandit}\label{alg:ucb1-bandit}
% \begin{algorithmic}[1]
% \For{$a \in A$}
%     \State $N_a = \epsilon$
%     \State $R_a = 0$
% \EndFor
% \For{$t=1,2,...,F$}
%     \State Select $a_t = \argmax_{a \in A} R_a + \frac{\sqrt{2log(t)}}{N_a}$
%     \State Observe reward $R_t$ for action $a_t$
%     \State $N_a = N_a + 1$ 
%     \State $R_a = R_a + \frac{R_t - R_a}{N_a}$
% \EndFor
% \State \textbf{return} $\argmax_{a \in A} R_a$
% \end{algorithmic}
% \end{algorithm}

% We show an example evaluation where we run the UCB1 and Uniform (sample all actions equally) bandit. Figure \ref{fig:bandit-search-strat} shows that the UCB1 bandits sample actions that generate a larger reward with higher probability than Uniform.


% \begin{figure}[!t]	
% 	\centering
% 	\includegraphics[width=4cm]{figs/bandit_reward/sample_dist.png}
% 	\includegraphics[width=4cm]{figs/bandit_reward/num_samples.png}
% 	\caption{Searching over replica action space with Uniform and UCB1 Bandit}
% 	\label{fig:training-reward}
% 	\vspace{-0.5cm}
% \end{figure}

%%% >>>>>>>>>>>>>


% \subsubsection{Effect of Optimizations on Search Time} We evaluate the benefits of training \sysname{} with the optimizations presented in this Section. We train \sysname{} with several ablations of the previously noted optimizations on two applications: Book Info and Online Boutique which consist of 4 and 11 microservices respectively (these applications are described in more detail in Section \ref{sec-evaluation}). First, we vary the service selection policy (presented in Section \ref{subsubsec:select-service}) to a memory utilization based selection where services requesting the most memory for a given workload are explored and a random service selection policy where the next service explored is selected uniformly at random. Additionally, we run training without the warm start introduced in Section \ref{subsubsec:warm-starting}. Lastly, we estimate training time without early stopping (introduced in Section \ref{subsubsec:greedyhillclimbing}) after reaching our latency target; to do so we simply document the maximum number of samples \sysname{} is configured to take before exiting. For all ablations, we document the number of samples and the median latency for the chosen configuration once training is concluded.

% All models are trained on four RPS values for one request distribution with a 50ms latency target. We find that without the optimizations presented \sysname{} takes 1.6x-12x the amount of samples to train Book Info and 1.58x-2.06x the amount of samples to train Online Boutique. In most cases, these ablations lead to policies which converge to a median latency above our target. These results are shown below in Tables \ref{tab:model-ablation-bi} and \ref{tab:model-ablation-ob}. Additionally, plots which show the reward, latency and instances used in training are shown in Appendix Figures \ref{fig:bi-training-trajectory-ablation} and \ref{fig:ob-training-trajectory-ablation}. 


% \begin{table}[H]
%   \begin{tabular}{lll}
%     \toprule
%     Training Setup& Num Samples & Latency \\
%     \midrule

%   \sysname{}&  50&  36.00  \\
%   \sysname{} - MEM service selection.   & 80 &  33.00 \\
%   \sysname{} - Random service selection & 190 &  35.75\\
%   \sysname{} - No Warm Start            & 270 & 265.75\\
%   \sysname{} - No Early Stopping        & 600 & - \\
  
%   \bottomrule
% \end{tabular}
% \caption{Search Ablations for Bookinfo Application}
% \label{tab:model-ablation-bi}
% % \vspace{-0.25cm}
% \end{table}

% \begin{table}[H]
%   \begin{tabular}{lll}
%     \toprule
%     Training Setup& Num Samples & Latency \\
%     \midrule

%   \sysname{}&  290&  47.00  \\
%   \sysname{} - MEM service selection.   & 460 &  172.25 \\
%   \sysname{} - Random service selection & 600 &  602.00\\
%   \sysname{} - No Warm Start            & 550 & 95.25\\
%   \sysname{} - No Early Stopping        & 600 & - \\
  
%   \bottomrule
% \end{tabular}
% \caption{Search Ablations for Online Boutique Application}
% \label{tab:model-ablation-ob}
% % \vspace{-0.25cm}
% \end{table}
% otherwise user defined policies for example.

==> old_text/evaluation.tex <==
% The first node pool, a monitoring node pool, contains the Istio and Prometheus microservices responsible for gateway logic, logging and monitoring of the application microservices. This node pool is fixed in size for all experiments with 3 \texttt{e2-highmem-8} (8 vCPU, 64GB MEM) instances and does not use autoscaling of any kind.

% Our second node pool contains microservices which contain our application containers. The application node pool autoscales dynamically based off of an autoscaling policy with the pool's total size upper bounded by the sum of replica range upper limits across our microservice. Each node in our application node pool is a \texttt{n1-standard-1} instance (1 vCPU, 3.75GB MEM).

% Each microservice within an application has a predefined minimum and maximum replica value. We hold these two values fixed for \sysname{} and all baselines during both training and evaluation time.

% All microservice replicas request 600 millicpu and 2400 MB of memory. Other resources that occupy significant compute and memory resources include a metrics agent deployed by Google Cloud as well as the Kubernetes proxy. Including the microservice replica and other resources, we leave on average a 4\% slack in allocatable CPU resources and 2\% slack in allocatable memory on each node. These settings are applied for \sysname{} and all baselines.

% On our managed Kubernetes cluster, we do not modify the default timeout set by the ingress gateway for Google Kubernetes Engine which allows requests to remain alive for up to 30 seconds.
% Double check this timeout.


% \as{What does cluster state refer to here?}
% \as{How are these 20K states related to the current workload?}

% For each microservice in an application we extract and concatenate the following variables to construct a feature vector: (1) the number of replicas for the microservice, (2) the logarithm of the microservice replicas, (3) the ratio of the workload's requests per second divided by the number of microservice replicas. Additionally we append a value which contains the total requests per second to the cluster. We define the observed reward, the target variable of our regression, as we do for \sysname{} in Equation \ref{equation:reward-function}. For all applications we randomly sample feature vectors from the set of possible choices. Given a sampled feature vector which constitutes a cluster state and workload in terms of request per second, we evaluate the reward to construct a training example. Once all training examples are collected, we train our ordinary least squares regression.

% During inference time, we randomly sample 20,000 possible cluster configurations and append the current requests per second to each sample to construct feature vectors. We use the trained linear regression model to predict the associated reward for each configuration and update our cluster to highest reward cluster configuration. We break ties by choosing the lowest cost configuration among tied candidates.


% For the smallest application which consists of a single microservice, Simple Web Server, we solve an optimal experiment design problem as presented in Ernest to select from the possible microservice configurations. For all other applications we find it infeasible to do so using CVXOPT ~\cite{cvx-opt:online} as solving the linear program associated with the optimal experiment design takes more memory than available on our 64GB RAM training machine. The second largest application, Book Info, contains 4 microservices and a replica range of 15 instances per service. This results in 202,500 ($15^4 \cdot 4$) possible training examples across 4 contexts and larger applications can expand the set of possible training examples combinatorially.

% Further, we modify the system presented in Ernest by using ordinary Least Squares Linear Regression rather than Non-Negative Least Squares, which lower bounds weights at 0. Since our reward, unlike the target variable in Ernest -- time taken to run a task -- can be negative, we allow weights to take on any positive or negative value.

% For all experiments except those on the Train Ticket application we set $w_i$ to 3 and $w_v$ to 1, which means we are willing to add a replica to a microservice given that it reduces the end to end latency by at least 3 milliseconds. On the Train Ticket application, we set both $w_i$ and $w_v$ to 1 as training failed to converge with a higher value for $w_i$.

% First, as we do not assume availability of low-level architecture specific information on CPU, Memory, I/O and network the context provided to our DQN is less rich than in FIRM. The features we provide to our DQN are requests per second as well as per-microservice CPU utilization, memory utilization and number of replicas. As in FIRM, we use a deep deterministic policy gradient algorithm ~\cite{lillicrap2015continuous}. However, we modify the output of the reinforcement learning model. In FIRM resource thresholds are produced which dictate scale up/down actions similar to the Kubernetes CPU and Memory autoscalers. For our evaluation, the DQN outputs a value between $[-1,1]$ which we map linearly to the minimum and maximum replica range for each service. Lastly, our evaluations depart from those in FIRM as we allocate only one microservice replica per machine and the size of our cluster is dynamic in response to the autoscaler policy. During inference time, we provide a context including the requests per second and per-microservice CPU, memory and replicas; we then allocate cluster resources based on the output configuration. 

% We adapt a DQN autoscaler inspired by FIRM ~\cite{qiu2020firm} which leverages a neural network based controller to manage microservices. We make a few modifications to this autoscaler based on our training and evaluation context.

% \subsection{Cluster Autoscaler} The CPU and memory threshold autoscaling baselines use a cluster autoscaler available in the Google Cloud Platform ~\cite{GKE:online}. All other policies are evaluated with the cluster autoscaler described in Section \ref{subsec:cluster-autoscaler}. We find similar performance across both cluster autoscalers

% whose service level objectives dictate a lag of up to 60 seconds for allocating instances for new cluster nodes ~\cite{kub-cluster-autoscaler:online}

% Based on the service level objectives, the time to allocate resources for new replicas of a service can range be up to 30 seconds for a small cluster and 60 seconds for a large cluster with an average time of 5 and 15 seconds respectively. Small clusters are defined as less than 100 VMs with 30 pods each and large clusters ranging from 100-1000 VMs ~\cite{kub-cluster-autoscaler:online}.


% For the BookInfo application, \sysname{} provides the most cost effective policy across all candidate autoscalers. The next cheapest policy (CPU-70) costs \textbf{28.5 \%} more. For the Online Boutique evaluation, we train and deploy two models. \sysname{}-50 has been trained to target a 50 ms median latency and \sysname{}-tail-100 has been trained to target a 100 ms 90\%ile latency. For 50 ms median latency and 100 ms tail latency targets respectively, the next closest autoscaling policy cost \textbf{51\%} and \textbf{34.3\%} more than what \sysname{} costs (seen in Figure \ref{fig:ob-fr}). For the Sock Shop application, we find that the most cost effective autoscaling policy depends on the workload (Figure \ref{fig:ss-constant-rate}). Overall, \sysname{} is the cheapest policy to meet the latency target across all workloads. On the Train Ticket application, we train and evaluate two \sysname{} policies, for 50 ms median latency and 100 ms 90\%ile latency, seen in Figure \ref{fig:tt-fr}. For 50 ms median latency, \sysname{} reduces cost by \textbf{30.1\%} compared to the next closest autoscaling policy. For tail latency evaluations, the closest autoscaling policy in terms of latency costs \textbf{20.8\%} more than \sysname{}.

% The Constant Rate evaluation results for the simple web server application are shown in Figure. \sysname{}-50 has trained on 1000 and 2000 requests per second with a 50ms median latency target and is asked to autoscale for these trained context as well as two unseen workloads.

% For the Simple Web Server application, \sysname{}-50 meets its median latency target on all four workloads run. It \textbf{matches the cost} of the closest median autoscaling policy -- 90\% CPU autoscaling.  we train \sysname{} on 200, 400, 600 and 800 requests per second with a target of 50ms median latency.

% Across applications, workloads, and latency targets the closest autoscaling policy to \sysname{} varies. This uncertainty in terms of which policy works best for a given setting indicates a key benefit of learning an autoscaling policy for particular workloads.

% For 200 requests per second, Linear Regression is the cheapest policy. For 300 requests per second \sysname{} and CPU-30 are the cheapest policies which meet the latency target and for 400 and 500 requests per second \sysname{} and Linear Regression use the same number of instances to meet the 50ms target. 

% On the Train Ticket application, we train and evaluate two \sysname{} policies seen in Figure \ref{fig:tt-fr}. Across a set of in and out of sample workloads, we find that \sysname{} meets the median latency target in 3 of 4 workloads while costing \textbf{30.1\%} less than the closest policy, CPU-30. For tail latency evaluation, we see that \sysname{} meets its target in 2 out of 3 evaluations with the closest policy CPU-30 costing \textbf{20.8\%} more than the price of \sysname{}.


% For the Simple Web Server application, \sysname{}-50 reduces cost over the next most cost effective policy by \textbf{35.5\%} and \textbf{32.4\%} for in and out of sample workloads respectively.  On the Book Info application, \sysname{} meets its latency target but is outperformed by the CPU-70 policy with a cost reduction of \textbf{-3\%} and \textbf{-7\%} for in and out of sample workloads respectively. For the Online Boutique application, \sysname{} reduces cost over the cheapest policy which meets the target, CPU-30, by \textbf{46\%} on the in sample workload. On the out of sample workload, \sysname{} meets the 50 ms latency target and reduces cost by \textbf{39.6\%}. For the Train Ticket application, \sysname{} performs worse on the in sample diurnal workload compared to the CPU-30 and CPU-70 policies. It incurs a cost reduction of \textbf{-7.4\%} with almost 2x the latency of the CPU-70 autoscaler. For the out of sample workload, \sysname{} is the most cost effective and only policy which meets the 50 ms latency target. \sysname{} reduces cost by \textbf{28.7\%} compared to CPU-30 which has the closest median latency to \sysname{}.

% In the Sock Shop application, \sysname{} reduces cost on In and Out of Sample diurnal workloads by \textbf{1.11$\times$} and \textbf{1.04$\times$}. The next cheapest policy is CPU-70.



% We analyze some of the decisions made by the bandit autoscaler and then detail the training cost for each application to understand the cost associated with performance improvements.

% We take a closer look at how \sysname{} scales microservices to reduce the cost of meeting median and tail latency targets for a few of our evaluated applications.

% % In this section, we try to understand the performance gains of COLA and shed light on why it works

% \paragraph{Median Latency} An important distinction that \sysname{} can make based on its experience is understanding which microservices reduce end to end latency significantly and which microservices do not. We take a closer look at scaling decisions made for the Book Info application. One primary difference seen in Figure \ref{bookinfo-allocation-plot} is that \sysname{}'s autoscaling policy chooses to only scale the \texttt{productpage} microservice even though CPU utilization is elevated in other services. 

% % \begin{figure*}[!t]

% % \end{figure*}


% First, for the Bookinfo Application \sysname{} meets its autoscaling target of 50ms median latency (serving requests with 38ms median latency) which means adding any additional instances would not improve the system's reward. In Figure \ref{scaling-effect-bi} we see that adding instances for other service improve the end to end latency marginally, do so beyond the latency target specified, and with less value than our tradeoff specified (in this case a latency reduction of 3ms per additional replica).

% \begin{figure*}[!t]

% %% first three subfigures
% \subfigure{%
% 	\label{bookinfo-allocation-plot}
% 	\includegraphics[width=8cm]{figs/analysis/allocations/bi_dist.pdf}
% }%
% \hspace*{\fill}
% \subfigure{
% 	\label{allocation-diff-ob}
% 	\includegraphics[width=8cm]{figs/analysis/allocations/ob_dist.pdf}
% }%
% \captionsetup{justification=centering}
% \caption{VM Allocations across Microservices for Book Info (left) and Online Boutique (right).}\label{scaling-allocations}

% %% first three subfigures
% \subfigure{%
% 	\includegraphics[width=8cm]{figs/updated/allocations/details_num_instances.png}
% }%
% \hspace*{\fill}
% \subfigure{
% 	\includegraphics[width=8cm]{figs/updated/allocations/reviews_num_instances.png}
% }%
% \captionsetup{justification=centering}
% \caption{Effect of Scaling 'Reviews' and 'Details' services on End to End Latency}\label{scaling-effect-bi}

% \subfigure{%
% 	\label{median-latency-endpoint-dist}
% 	\includegraphics[width=8cm]{figs/updated/endpoint_dist/cola_median_latency_endpoint_dist.png}
% }%
% \hspace*{\fill}
% \subfigure{
% 	\label{tail-latency-endpoint-dist}
% 	\includegraphics[width=8cm]{figs/updated/endpoint_dist/cola_tail_latency_endpoint_dist.png}
% }%
% \captionsetup{justification=centering}
% \caption{Online Boutique \sysname{}-50ms and \sysname{}-tail-100ms Latency by URL}\label{fig:lat-by-url-ob}

% \end{figure*}


% \paragraph{Tail Latency} \sysname{} trained to optimize 90th \%ile tail latency has comparable median latency with \sysname{} trained for median latency for the Online Boutique application. However when trained to explicitly optimize tail latency, we see tail latency is reduced by close to 50\%.

% Based on the allocation differences shown below in Figure \ref{allocation-diff-ob} the primary difference between the two trained systems is that \sysname-tail-100 aggressively scales up the \texttt{cartservice} microservice in our application.



% \begin{figure*}[!t]
% %% first three subfigures
% \subfigure{%
% 	\label{median-latency-endpoint-dist}
% 	\includegraphics[width=8cm]{figs/updated/endpoint_dist/cola_median_latency_endpoint_dist.png}
% }%
% \hspace*{\fill}
% \subfigure{
% 	\label{tail-latency-endpoint-dist}
% 	\includegraphics[width=8cm]{figs/updated/endpoint_dist/cola_tail_latency_endpoint_dist.png}
% }%
% \captionsetup{justification=centering}
% \caption{Online Boutique \sysname{}-50ms and \sysname{}-tail-100ms Latency by URL}\label{fig:lat-by-url-ob}
% \end{figure*}

%   4. COLA tailors its policy to the latency objective of interest. Tail instead of median latency.


==> old_text/implementation.tex <==

% \begin{algorithm}
% \caption{\sysname{} Inference Procedure}\label{alg:scalecluster}

%   \begin{algorithmic}[1]
%     \BlankComment{}
%     \Function{scaleCluster}{$C_{obs}, W_{train}, C_{train}, S_{train}$}
%     \For{$c \in C_{train}$}\Comment{Iterate over trained cluster workloads.}
%         \State $N_a = \epsilon$ \Comment{Number of times state $a$ is sampled.}
%         \State $R_a = 0$ \Comment{Average reward for state $a$.}
%         \State $L_a = 0$ \Comment{Average latency for state $a$.}
%     \EndFor
%     % \LineCommentCont{Observe reward for each action and update average rewards.}
%     \For{$t=1,2,...,F$}
%         \State $a_t = \argmax_{a \in A} R_a + \frac{\sqrt{2log(t)}}{N_a}$ \Comment{Action for trial $t$.}
%         \State Update cluster replicas based on action $a_t$
%         \State Compute total replicas/VMs $M$ used for action $a_t$
%         \State Observe latency $L_t$ for action $a_t$
%         \State $R_t = min((l_{target} - L_t), 0) - M \cdot w $
%         % \State Observe reward $R_t$, latency $L_t$ for action $a_t$
%         \State $N_{a_t} = N_{a_t} + 1$ 
%         \State $R_{a_t} = R_{a_t} + \frac{1}{N_{a_t}} (R_t - R_{a_t})$
%         \State $L_{a_t} = L_{a_t} + \frac{1}{N_{a_t}} (L_t - L_{a_t})$
%     \EndFor
%     \State $a_{opt} = \argmax_{a \in A} R_a$ \Comment{Get action with highest reward.}
%     \State $l_{opt} = L_{a_{opt}}$ \Comment{Get corresponding latency.}
%     \State \textbf{return} $a_{opt}, l_{opt}$
%     \EndFunction
%   \end{algorithmic}
% \end{algorithm}

%% >>>>>>>>>>>>>>>

% Lastly, we aggregate the cluster states for all similar workloads by their Euclidean distance.
% For each deployment, $i$, in our microservice, we scale the number of replicas to $\lceil \hat{S}_i \rceil$.
% For each workload, we compute a linearly interpolated state, $\hat{S}$ between the two training context. For each deployment, $i$, in our microservice, we scale the number of replicas to $\lceil \hat{S}_i \rceil$. \footnote{Another approach to perform this inference is to use a linear contextual bandit, which builds a linear regression model on a set of trained context (discussed in Section \ref{subsec:lcb-v-i})}

% $$    \hat{S} = \frac{d_1 \cdot \hat{S}_{1} + d_2 \cdot \hat{S}_{2}}{d_1 + d_2} $$

% Once we finish training, we have a set of context that span the request per second range that a developer expects their application to encounter. At inference time, our metrics agent computes the current context, $C_{obs}$, after which we place this vector between an upper and lower trained context, $C_{upper}, C_{lower}$ for inference. We weight how close the observed context is to these two training points. For example for the distance to the upper context: $d_{upper} = | C_{obs} - C_{upper} |$

% Then, we compute a linearly interpolated state, $\hat{S}$ between the two training context. For each deployment, $i$, in our microservice, we scale the number of replicas to $\lceil \hat{S}_i \rceil$. \footnote{Another approach to perform this inference is to use a linear contextual bandit, which builds a linear regression model on a set of trained context (discussed in Section \ref{subsec:lcb-v-i})}


% \begin{equation}
% \label{eq:interpolate-workload}
% \hat{S} = \frac{d_{lower}\cdot S_{lower} + d_{upper}\cdot S_{upper}}{d_{lower} + d_{upper}}
% \end{equation}


% \Para{Request Distribution Generalization} During inference, we may be faced with a request distribution different from those seen during training. Some request operations may receive unusually high or low requests if user behavior in an application changes, for example.

% Rewrite this as a context rather than the state itself.





% Request count/distribution cases for generalization

% Interpolation Procedure

% Request Distribution Generalization

% Figure describing Procedures

==> old_text/intro.tex <==

% as microservices become segmented
% becomes challenging for two reasons - can not apply same autoscaling policy to all metrics
% Each service can not capture the effect of the service as a whole
% For instance - backpressure

% 1. Intro to microservices
% 2. Autoscaling hard for these reasons
% 3. Some effects from 
% However, this flexibility and modularity comes at a cost: complexity in resource management. As applications move from monoliths to microservices, three challenges arise in the automatic scaling of compute resources allocated to each microservice within an application. First, each microservice often needs to be scaled differently depending on how complex its application logic is \cite{gan2020unveiling}. Second, traditional autoscaling strategies based on CPU or memory utilization thresholds are difficult to configure because the right value of these thresholds can vary with time. Third, while microservices promote the ability to rapidly iterate on code, adding a feature or fixing a bug in one microservice can lead to changes in the workload experienced by microservices downstream from that microservice \cite{zhang2021sinan}. This change in workload, in turn, affects, the scaling of all downstream microservices \cite{gan2018architectural}.

% Issues with current approaches
%Such an architecture 
%Building applications under a microservice architecture has gained wide adoption in recent years and such architectures now serve some of the largest web applications in the world such as Netflix \cite{netflix-ms:online}, Twitter \cite{twitter-ms:online} and Uber \cite{uber-ms:online}. These applications are written such that monolithic codebases are broken down into several smaller microservices, each exposing endpoints for code execution.


% by monitoring the workloads a cluster receives and subsequently scales microservices 

% Generally as services are more replicated latency decreases but cost increases for microservice applications. 


% and the number of VMs in our cluster. \sysname{} is built to introduce minimal dependencies for developers, and in our deployments, \sysname{} only assumes dependence on functionality widely available through Kubernetes and major cloud providers. 


% Given upper and lower bounds for the number of VMs for each microservice, \sysname{} explores the set of possible VM allocations to each microservice under a multi-armed bandit framework in order to select a configuration for each workload that optimizes our reward. We show that this optimization can be accomplished using an alternating maximization of our reward metric across the different microservices in an application. Further, we show how to prioritize the exploration of services which disproportionally and negatively impact our reward metric. Once training is completed, 

% It relies on a machine learning model that maps workloads seen at an application frontend to the allocation of compute resources to various different microservices forming the application. This model aims to meet end-to-end latency targets (across all microservices touched by a request to the application) while minimizing the dollar cost of running the entire application on the public cloud.


% Lastly, we delve deeper into some of the resource management decisions \sysname{} makes when optimizing latency to understand how \sysname{} allocates resources. Additionally, we evaluate the economics of using \sysname{} to allocate resources and demonstrate how the cost associated with training can be amortized quickly for our evaluated applications. We note failure cases including taking measurements which may be noisy, encountering unseen and unexpected workloads, and selecting model hyperparameters. For these potential failure cases, we explain how \sysname{} can be made robust. 

%     \item Introduction to microservice deployments - simplicity in collaboration, complexity in management
%     \item Current approaches to autoscaling microservice clusters - cpu based autoscaling and other threshold based techniques
%     \item Learned approaches to solve system problems (specifically qoe/control and rl/bandit)
%     \item The approach we take along with key design decisions - simple models, metrics that effect users+developers, scalable training methods
%     \item Summary of results and organization of paper
% \end{enumerate}

% Note - use \paragraph instead of 

==> old_text/related.tex <==
  %Cluster autoscaling adjusts the number of virtual or physical machines a microservice uses. It is a generally available feature from some cloud providers including EKS Cluster Autoscaler in AWS ~\cite{ClusterA11:online}, GKE Cluster Autoscaler in Google Cloud Platform ~\cite{Clustera68:online}, and AKS Cluster Autoscaler in Microsoft Azure ~\cite{Usethecl21:online}. Our main contribution is developing a horizontal pod autoscaling system but we also develop a simple cluster autoscaler to deploy \sysname{} as a standalone solution for settings where a cluster autoscaler is not available. In Section \ref{subsec:coexistence-noca} we show evaluations of the coexistence of \sysname{}'s horizontal pod autoscaler with the GKE cluster autoscaler.

%Also building on fine grained microservice logs, techniques to provide predictive alerting and diagnosis of performance issues and failures is a subject of recent work. Such systems have been developed for predicting  quality of service (QoS) violations ~\cite{gan2019seer, delimitrou2013paragon, chen2019parties, patel2020clite}.

% \textbf{Logging, Monitoring, and Diagnostics} Given the complexity and scale of modern microservice deployments~\cite{gan2020unveiling}, a wide body of research has been performed on how to log microservices at a fine grained level. Such logging platforms afford users the data to trace requests as they travel through large microservice graphs including Dapper ~\cite{sigelman2010dapper}, Zipkin ~\cite{OpenZipk7:online}, Jaegar ~\cite{Jaegerop26:online}. Adaptive sampling techniques have also been developed to assist in scaling the collection of logs in large clusters such as Sifter ~\cite{las2019sifter} and work by Las-Casas et. al ~\cite{las2018weighted}. 

% Leveraging these fine grained traces of requests through a microservice log, systems have been created for application performance monitoring (APM) including AppDynamics ~\cite{The1fast42:online}, SignalFx ~\cite{RealTime59:online}, Datadog ~\cite{CloudMon59:online}, NewRelic ~\cite{NewRelic3:online}, and LightStep ~\cite{httpslig99:online}. These systems help users track the performance of microservice cluster at the levels of compute resources, requests and individual spans of requests. Users are able to isolate performance issues across these levels through various visualization and querying capabilities embedded within APM systems.

% In Autotune ~\cite{chang2021autotune}, the authors propose a method similar to ours where latency impacted microservices are identified and scaled to meet resource requirements. Unlike \sysname{}, Autotune does not explicitly optimize a cluster for a specific performance target but rather aims to improve on a baseline microservice configuration. 

==> todo.tex <==
TODO:
1. Remove learned from several contexts where it is still used.
2. Explicit example of workload.
3. Paper has two main ideas: one is architectural (centralized vs. distributed autoscalers) and the second is algorithmic (use of utilizaion, spec. CPU utilization, as the microservice selection strategy). Need to emphasize this somewhere.
4. Appendix 8.9 references Figure 8 in the main body of the text, not sure if that's intentional.
5. Reference Equations in main body
6. Try to get all of the COLA pseudocode on one page like page 5 of the Raft paper: https://www.usenix.org/system/files/conference/atc14/atc14-paper-ongaro.pdf
7. Prevent spillover in appendix. Fix formatting in the appendix more generally.

To Do:
------

2. **\- Page 4 (Sec. 3.1): I found the interchangeable usage of context and workloads confusing. It helps to use a single term, after an initial clarification.**
   - Fix this wording



Done
1. For Table 1, some description of the methodology is needed. It was a bit difficult to put these cost reduction numbers into appropriate contexts
2. A key component of your training algorithm is to select the microservice with "highest increase in CPU utilization understand current workload" (page 4). I have a hard time to figure out what the reference point is when computing this increase.
3. "based autoscalers which receive a similar level of application information as COLA." Could you cite / describe the other autoscalers?**
4. Table 1 - could you specify the cost reduction is with respect to what baseline?**
5. Autopilot system related work
6. Tabular data remove latency not compared against (9:10-9:40)
1. **- Page 3 (Sec. 3 first para): why limit to a single pod per VM? Even when a tenant pays for VM, the tenant may start multiple pods on the same VM.**
   - Started, need to rephrase this portion potentially reorganize where this appears
3. **- Page 5: Equ (1). The model appears to be simple and can be more general, say instead of simple M, it can use a pricing model of VMs.**
   - Talk about this to an extent -> with homogenous VMs we do x. When operating in seperate cases, we discuss the modified cost function in appendix
4. **Would be good to specify how long you run the workloads for?**
   - Add this detail

7. **I appreciate that you also tested against other machine-learning-based policies, but I did not gain insight into why these other strategies did not perform as well as your multi-armed bandit approach. That might be worth exploring should you revise the paper.**
   - Talk about training cost needed
     - Maybe show how long DQN etc would have to be trained to perform at a similar level to COLA
6. **The training costs do look reasonable except for one or two applications and their workloads. How about RL inference cost? Are they negligible? It might be helpful to add some analysis or summarized experimental results.**
   - Not clear this is needed/relevant
5. **- For example, it took me a while to try to figure out whether you train a single model for all contexts (workloads) or you train one model for each one of a given set of contexts. The former is clearly more interesting but I understand that it is second. It helps if this is specified fully.** 
   - Add full pseudocode (short version in paper and longer in appendix)
   









-----------------------------------------




Major:
1. Say number of workloads and how they have been broken down into various types.
2. Increase font sizes on the figures.

Minor:
2. Don't bother with references to paragraphs.
3. endpoint vs. request distribution.
4. Maybe we can remove the term workload vector? We don't really use it anywhere.
11. requests vs. limits
9. comma after and consistently (or not).
5. Use VM instead of replicas/pods/instances/nodes; but do define pods and nodes at the beginning.
12. Write numerals as numbers (2) and not alphabets (two) so that they stand out. (I know that's not standard, but it helps make things visible.)
13. Use ~\cite and not \cite.
15. utilization threshold not utilization target.
19. We should be using --- (emdash) instead of -- (endash).
31. There must be a space between number and unit (50 ms, not 50ms).
-------------------------------------------

% Run Evaluations
10. More retraining examples
31. Run more out of distribution examples

% Other
13. Discuss networking problem in Intro
14. Discuss compute congestion effect (with tracing data)
17. Add information on complexities of applications - dynamic microservice paths
18. Model intro off of flood intro -- need for workload, application codesign for autoscalers

% Maybe
16. Convex objective -- can this be shown


DONE
-------------------------------------------

23. Modify algorithm to simplify select service fn
7. Section 4, 1 line comments for code
6. Check for operation name -- update any other type of reference
21. Balance bib
20. Move to Sigcomm format
9. Change model ablation name
22. Check for broken fig/table references
8. Future work - more efficient ways to search
11. Example applications - TT largest application in terms of # of microservices available as open source software
23. Fix Space Factor issue
18. Cycles in DAG -- do not mention in Background
1. Cleanup section 2.1
2. Cleanup section 2.2
15. Implement Binary search version of COLA (start a few runs to evaluate -- for BI)
25. Implement tracing for OB based on Jessica's code
26. Export traces to database
% Evaluation Writing
19. Comparison with other ML models -> Add plots into main body.
12. Interpretability - need to address this one. Add in data from appendix.
30. Open API Spec add link
28. Binary Search train all applications
3. Simplify writing for HPA shortcomings (Section 2.3)
30. Change to 1 hyperparameter for reward
4. Recreate plots for Section 2.3
27. Plot effect of autoscaling with tracing view
5. Definitions in Section 2.4 itself for reward/objective and procedure
29. Outer outer loop for algorithm with hyperparameter selection


-------------------------------------------
Addressed Above:
[x] 0
[x] 1
[x] 2
[ ] 3
[x] 4
[x] 5
[x] 6
[x] 7

-------------------------------------------
0. For a SIGCOMM submission (and more generally as well), focusing the
paper on the *networking* aspect of the problem would help. There is
an overlay network of microservices, which is formally a network of
queues, where queueing delays arise out of compute congestion (see
point 5). Our goal is to keep such compute congestion low by deploying
resources ahead of time. Might even help to distinguish this from the
network's canonical resource allocation problem: congestion control.
In congestion control, the resources are almost always fixed, whereas
the main knob we have here is to deploy more resources as needed. In a
sense, our work is closer to how real queueing models in the world
work (where you eventually need to add additional capacity) rather
than queueing in the context of networking, where capacity is always
fixed.

1. Better comparison to some version of Autopilot for our setting: at
the outset, their setting is different from ours (reducing slack vs.
reducing dollars). But maybe we can adapt their algorithm to our
dollars setting and see how they compare to us?

2. Motivating the need for a data-driven approach to autoscaling:
Section 2 already does some of this with the queuing theory models,
but we should sharpen this. Maybe we can reduce the math and increase
the intuition. We could add some quantitative comparisons to a naive
policy (e.g., the Kubernetes CPU-threshold-based autoscaler) right
here in section 2. This might help with answering "why learning" or
more specifically "why contextual bandits"

3. Handling stateful services: This is not something I had explicitly
thought of. Increasing the number of replicas could (in theory) hurt
latency by increasing synchronization overhead for stateful services.
This is something we should discuss.

4. Dynamic microservice paths: What if the next microservice is a
function of the RPC response from a previous microservice? I don't
think our current setting handles this.

5. Definitions: What is the *graph* in our context? What does a node
correspond to? Where do queues build up? And why? It's useful to
stress that the queue build up is due to the *computational work* of
responding to RPCs, and does not arise from one-way delays in the
network or queues in physical switches. This paper
(http://www.abelay.me/data/shenango_nsdi19.pdf) uses the term compute
congestion to refer to a similar context and we could repurpose it for
COLA as well.

6. Cycles in the DAG: Not sure what these mean in our context? Maybe
our problem definition makes these impossible? It would be good to
address these head on.

7. DeathStarBench: Again would be useful to address whether we can or
can't use this suite head on.


